Data Traceability for Privacy Alignment

This paper offers a new privacy approach for the growing ecosystem of services -- ranging from open banking to healthcare -- dependent on sensitive personal data sharing between individuals and third parties. While these services offer significant benefits, individuals want control over their data, transparency regarding how their data is used, and accountability from third parties for misuse. However, existing legal and technical mechanisms are inadequate for supporting these needs. A comprehensive approach to the modern privacy challenges of accountable third-party data sharing requires a closer alignment of technical system architecture and legal institutional design. In order to achieve this privacy alignment, we extend traditional security threat modeling and analysis to encompass a broader range of privacy notions than has been typically considered. In particular, we introduce the concept of covert-accountability, which addresses the risk from adversaries that may act dishonestly but nevertheless face potential identification and legal consequences. As a concrete instance of this design approach, we present the OTrace protocol, designed to provide traceable, accountable, consumer-control in third-party data sharing ecosystems. OTrace empowers consumers with the knowledge of who has their data, what it is being used for, what consent or other legal terms apply, and whom it is being shared with. By applying our alignment framework, we demonstrate that OTrace's technical affordances can provide more confident, scalable regulatory oversight when combined with complementary legal mechanisms.

==> Makefile <==
INPUTNAME=main
PAPERNAME=paper
TEXFILES = $(wildcard *.tex) $(wildcard *.sty) $(wildcard bibs/*.bib) $(wildcard sections/*.tex)
FIGURES = $(wildcard figures/*.tex) $(wildcard figures/*.tikz) $(wildcard figures/*.gnu)
GRAPHICS = $(wildcard graphics/*.pdf) $(wildcard graphics/*.png)
LISTINGS = $(wildcard listings/*.tex)
BUILD=./build
LATEX_CMD=pdflatex
LATEX_FLAGS=-output-directory=$(BUILD) -aux-directory=$(BUILD) 
DEPENDENCIES = $(TEXFILES) $(FIGURES) $(GRAPHICS) $(LISTINGS)

# Default to compile when no specification is provided:
all: $(BUILD)/$(PAPERNAME).pdf

pdf: $(BUILD)/$(PAPERNAME).pdf

$(BUILD)/$(PAPERNAME).pdf: $(DEPENDENCIES)
	mkdir -p $(BUILD)
	$(LATEX_CMD)  $(LATEX_FLAGS) $(INPUTNAME).tex < /dev/null
	bibtex $(BUILD)/$(INPUTNAME).aux
	$(LATEX_CMD) $(LATEX_FLAGS)  $(INPUTNAME).tex < /dev/null
	$(LATEX_CMD) $(LATEX_FLAGS)  $(INPUTNAME).tex < /dev/null
	mv $(BUILD)/$(INPUTNAME).pdf $(BUILD)/$(PAPERNAME).pdf

henry:
	latexmk -pdf -pvc -latexoption=-halt-on-error \
		-latexoption=-file-line-error \
		-latexoption=-interaction=nonstopmode \
		-latexoption=-synctex=1 $(INPUTNAME).tex || ! rm -f $(BUILD)/$(PAPERNAME).pdf

tar:
	tar --ignore-failed-read -cvzf $(PAPERNAME).tgz $(DEPENDENCIES) Makefile

clean:
	rm -rf $(BUILD)



==> sections/notes.tex <==
\subsubsection{The case for traceability regulation}

We contend that traceability regulation is a justified response to the digital services market's failure to adopt responsible data practices. In economic terms, market failure occurs when goods and services in a free market are allocated inefficiently, failing to maximize overall welfare. In the digital services context, these inefficiencies can manifest as privacy harms. In such cases, regulation may act as a corrective measure, offering protections that the marketplace cannot.
\djw{probably some citation to Acquisti and to privacy law review literature}

\subsubsection{Correcting privacy externalities and transaction costs}
Traceability regulation can bridge the gap between the ``price'' of a digital service and the full societal costs associated with its development and use. In an unregulated market, just as the price of steel, for example, does not account for the environmental harms caused by its production, the price of a digital service, i.e., the value of the data consumers ``pay'' to use the service, does not reflect the privacy harms that may result from the service provider's lax data practices. These ``externalities'' fall outside the economic considerations of the involved parties and are not borne by either the service provider or consumers. If consumers were to internalize these costs, such as by paying for identity theft protection in the event of a data breach, the cost of the digital service would rise, potentially leading to a reduction in its development and use. However, because these costs remain externalized, privacy harms persist at higher levels than they otherwise might. Since the marketplace alone cannot drive more responsible data practices, regulatory intervention may be warranted.

An alternative, Coasian view suggests that traceability regulation can correct for ``transaction costs'' between service providers and consumers. In this view, privacy harms arise not only from the service provider's lax data practices but also from the consumer's willingness to share their data with the provider in exchange for the convenience or enjoyment the service provides. While an efficient outcome could be achieved if both parties could bargain costlessly to reach a mutually preferred solution, the presence of transaction costs---costs associated with coming together to reach an agreement---prevents such bargains from taking place. In other words, although the service provider and consumer could agree to share the cost of reducing privacy harms through traceability, the impracticality of bargaining due to transaction costs makes such agreements improbable. Regulation, therefore, serves as a mechanism to correct this market inefficiency.

\subsubsection{Addressing privacy's collective action problem}

Traceability regulation can address privacy's collective action problem. When service providers act in their rational self-interest, such as by adopting lax data practices to improve their bottom lines, they increase the risk of privacy harms. These harms could be mitigated through mutual cooperating in providing traceability as a public good---goods that are nonrivalrous (one consumer's use does not diminish its availability to others) and nonexcludable (it benefits a group of people, and no individual or subgroup can be easily excluded from enjoying it). However, markets often struggle to produce public goods due to high transaction costs and the free-rider problem, where individuals are reluctant to contribute because the benefits primarily accrue to others, and they hope to benefit from others' efforts without contributing themselves. Traceability regulation, therefore, acts as a form of mutual cooperation to provide a public good that the market alone cannot effectively supply.

\subsubsection{Addressing privacy's information asymmetry problem}
Traceability regulation is not only justified by privacy's information asymmetry problem, but is also the solution to it. For a competitive digital services market to operate efficiently, consumers need sufficient information to evaluate competing services, particularly their data practices. When consumers lack transparency into how their data is handled, the market may fail to deliver optimal outcomes when it comes to privacy. Traceability information, like any commodity, is subject to supply and demand, but the market for traceability may be imperfect. First, while consumers collectively benefit from traceability, there may be no effective mechanism for them to share the costs of obtaining it. This can lead to a free-rider problem, where individual consumers hesitate to push for traceability support that would benefit everyone, thereby leaving everyone in the dark regarding providers' data practices. Second, digital services can be so complex that evaluating their risks requires expert analysis. Consumers may not be aware of the privacy risks associated with certain types of services. Third, even when providers voluntarily disclose traceability information to build consumer trust, their efforts may fall short if consumers are not paying close attention. In these cases, the market alone cannot ensure that consumers have access to the information they need.

\kl{TODO: Behavioral economics and bounded rationality: Consumers often make decisions that are not entirely rational due to cognitive biases or a lack of understanding about the long-term consequences of sharing personal data. Companies may exploit these biases by designing services that nudge users into agreeing to terms that are not in their best interest, such as overly broad data-sharing agreements. This manipulation exacerbates the inefficiency in resource allocation, as consumers' actual preferences regarding privacy are not reflected in their choices.}

%Government regulation is justified when (1) providers mislead consumers whose available legal remedies are expensive or impractical; (2) consumers cannot readily evaluate the information available; or (3) providers fail to furnish the information needed or demanded. In the last instances, the government may require providers to supply the information, just like financial disclosures mandated by the Securities and Exchange Commission (SEC) or risk disclosures required by the Occupational Safety and Health Administration (OSHA).

%First, it addresses the high ``transaction costs'' between controllers and consumers. From a Coasian perspective~\cite{}, privacy harms arise not only from controllers' lax data practices but also from consumers' willingness to exchange their data for services. While an efficient outcome could be achieved if both parties could bargain costlessly to reach a mutually preferred solution, the presence of transaction costs---costs associated with coming together to reach an agreement---prevents such bargains from taking place. In other words, although the controller and consumer could agree to share the cost of reducing privacy harms through traceability, the impracticality of bargaining due to transaction costs makes such agreements improbable. Regulation, therefore, steps in to resolve this inefficiency.
%In theory, an efficient outcome could be achieved if both parties could bargain costlessly and agree to share the costs of traceability. However, the existence of transaction costs make such agreements impractical. Regulation steps in to resolve this inefficiency.

%Beyond the legal framework, the very process of implementing and maintaining traceability systems can serve as an effective form of internal accountability. Support for traceability forces companies and developers to scrutinize their own data practices, fostering a culture of consciousness and care in how data is used. Even if formal enforcement does not occur immediately, the mere act of requiring companies to document and report their data practices can lead to self-regulation, as developers and data controllers become more aware of the potential risks associated with non-compliance.

%\subsection{Decreasing legal and technical costs}
%
%\subsubsection{Technical costs}
%
%\subsubsection{Legal costs}
%
%``Sunstein identifies three critical factors that influence the choice between rule-bound and individualized approaches:
%
%Decision costs: Rule-making requires extensive work before application, but individual discretion requires more effort at the point of decision. Rule-bound systems can reduce decision costs for legal authorities, while individualized systems may lead to higher costs in evaluating each case.
%
%Error costs: Rule-bound systems can reduce errors by offering clarity, but they may also lead to injustices if the rules are too rigid. Individualized approaches may mitigate errors in specific cases but increase the risk of inconsistency and subjectivity.
%
%Planning costs: Rules make it easier for people to plan their actions, as the rules are known in advance. Unclear or flexible rules can make planning more difficult and create uncertainty about legal obligations.''
%
%\subsection{Surveillance Concerns}



\header{Legal barriers to traceability}

Despite the promise of consumer agents, powerful incumbents, such as tech platforms and financial institutions, have frequently erected legal barriers to third-party data access. One of the most notable examples is the use of the Computer Fraud and Abuse Act (CFAA) of 1986. Originally designed to prevent unauthorized access to computer systems, the CFAA has been wielded by platforms like Facebook to stifle innovation by criminalizing data collection, even when consumers have consented. This tactic has been used to suppress third-party developers who create tools that challenge platform business models.

Fortunately, legal perspectives on these issues are shifting. In recent years, courts have begun to reverse earlier rulings that allowed incumbents like Facebook to use the CFAA to block third-party access. This shift reflects a growing recognition that consumers should have the right to share their data with third parties and that platforms should not be able to stifle innovation through legal threats. This evolving legal landscape provides a foundation for future reforms that could protect traceability agents from similar legal challenges.

Moreover, the Consumer Financial Protection Bureau's (CFPB) open banking rulemaking offers a promising model for how regulators can ensure consumer access to data. CFPB rulemaking has mandated that financial institutions must provide API access to third-party digital helpers. This rule ensures that consumers can access their financial data in a machine-readable, low-cost format, enabling personalized services and fostering competition.

\header{Holding the agents accountable}




==> sections/penalties.tex <==
\section{FTC Privacy Enforcement Penalties}
\label{sec:penalties}

\begin{table*}[h!]
\centering
\begin{tabular}{llrrr}
\toprule
                    Company (Parent) &       Date &  Penalty (in thousands) &  Revenue (in millions) &  Percent of Revenue \\
\midrule
Facebook, Inc. (Meta Platforms Inc.) & 2019-07-24 &         5000000 &  70697.0 &                   7.07 \\
          Google LLC (Alphabet Inc.) & 2019-09-04 &          170000 & 160743.0 &                   0.11 \\
                          Amazon.com & 2023-05-31 &           25000 & 574785.0 &                   0.00 \\
         Google Inc. (Alphabet Inc.) & 2012-08-09 &           22500 &  50175.0 &                   0.04 \\
                           Microsoft & 2023-06-05 &           20000 & 211915.0 &                   0.01 \\
      ChoicePoint, Inc. (RELX Group) & 2006-01-26 &           15000 &   1055.0 &                   1.42 \\
               Ring LLC (Amazon.com) & 2023-05-31 &            5800 & 574785.0 &                   0.00 \\
                  TikTok (ByteDance) & 2019-02-27 &            5700 &  17150.0 &                   0.03 \\
          Playdom Inc. (Walt Disney) & 2011-05-12 &            3000 &  88898.0 &                   0.00 \\
                      DIRECTV (AT\&T) & 2009-04-16 &            2310 & 122513.0 &                   0.00 \\
              WW International, Inc. & 2022-03-04 &            1500 &   1040.9 &                   0.14 \\
        Sony BMG Music Entertainment & 2008-12-11 &            1000 &  78880.0 &                   0.00 \\
                       Comcast Corp. & 2009-04-16 &             900 &  35756.0 &                   0.00 \\
          Experian Consumer Services & 2023-08-14 &             650 &   6620.0 &                   0.01 \\
                          Yelp, Inc. & 2014-09-17 &             450 &    377.5 &                   0.12 \\
            Iconix Brand Group, Inc. & 2009-10-20 &             250 &    232.1 &                   0.11 \\
      Kohl's Department Stores, Inc. & 2020-06-10 &             220 &  19974.0 &                   0.00 \\
           Hershey Foods Corporation & 2003-02-27 &              85 &   4173.0 &                   0.00 \\
                      Looksmart Ltd. & 2001-04-19 &              35 &     83.0 &                   0.04 \\
\bottomrule
\end{tabular}
\caption{Penalties as a Percentage of Revenue (Penalty in Thousands, Revenue in Millions)}
\end{table*}


